Unifi3D: A Study on 3D Representations for Generation and Reconstruction in a Common Framework

Following rapid advancements in text and image generation, research has increasingly shifted towards 3D generation. Unlike the well-established pixel-based representation in images, 3D representations remain diverse and fragmented, encompassing a wide variety of approaches such as voxel grids, neural radiance fields, signed distance functions, point clouds, or octrees, each offering distinct advantages and limitations. In this work, we present a unified evaluation framework designed to assess the performance of 3D representations in reconstruction and generation. We compare these representations based on multiple criteria: quality, computational efficiency, and generalization performance. Beyond standard model benchmarking, our experiments aim to derive best practices over all steps involved in the 3D generation pipeline, including preprocessing, mesh reconstruction, compression with autoencoders, and generation. Our findings highlight that reconstruction errors significantly impact overall performance, underscoring the need to evaluate generation and reconstruction jointly. We provide insights that can inform the selection of suitable 3D models for various applications, facilitating the development of more robust and application-specific solutions in 3D generation. The code for our framework is available at https://github.com/isl-org/unifi3d.

==> Figures/doctree_ablation_tables.tex <==

\begin{table*}[ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllll}
\toprule
Method & t(transform) & t(encode) & t(decode) & t(mesh) & Latent size & F-score $\uparrow$& CD (*1e-4) $\downarrow$\\
\midrule
DualOctreeGNN & 0.231 & 0.044 & 0.067 & 0.626 & 512 & 97.705 $\pm$ 2.126 & 24.925 $\pm$ 4.843 \\
DualOctreeGNN+VAE & 0.214 & 0.046 & 0.067 & 0.539 & 512 & 95.993 $\pm$ 2.259 & 29.89 $\pm$ 4.326  \\

DualOctreeGNN+VAE+KL & 0.139 & 0.042 & 0.063 & 0.442 & 512.0 & 76.487 $\pm$ 14.695 & 70.49 $\pm$ 31.301  \\
DualOctreeGNN+VQVAE & 0.142 & 0.053 & 0.07 & 0.464 & 512.0 & 79.528 $\pm$ 13.449 & 62.654 $\pm$ 23.726  \\
DualOctreeGNN+VQVAE+VQ & 0.136 & 0.055 & 0.071 & 0.466 & 512.0 & 85.876 $\pm$ 8.975 & 49.953 $\pm$ 15.639  \\

\bottomrule
\end{tabular}
}
\caption{Reconstruction quality (Category: Airplane, Dataset: ShapeNet test set) This shows that only AE and VAE have relatively better reconstruction quality with smaller std. \todo{Can we merge this Table and the following with Table 4?}}
\label{tab:reconstruction_dualoctree_loss_ablation}
\end{table*}

\begin{table*}[ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllll}
\toprule
Method & t(transform) & t(encode) & t(decode) & t(mesh) & Latent size & F-score $\uparrow$& CD (*1e-4) $\downarrow$\\
\midrule
DualOctreeGNN+AE & 0.166 & 0.032 & 0.065 & 0.622 & 512.0 & 88.88 $\pm$ 4.62 & 43.03 $\pm$ 7.702  \\
DualOctreeGNN+VAE & 0.226 & 0.033 & 0.067 & 0.692 & 512.0 & 90.114 $\pm$ 4.025 & 38.418 $\pm$ 6.962 \\


\bottomrule
\end{tabular}
}
\caption{Reconstruction quality (Category: Car, Dataset: ShapeNet test set) This shows that for cars, VAE outperforms AE for reconstruction for different categories.}
\label{tab:reconstruction_dualoctree_car}
\end{table*}


\begin{table*}[ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllll}
\toprule
Method & t(transform) & t(encode) & t(decode) & t(mesh) & Latent size & F-score $\uparrow$& CD (*1e-4) $\downarrow$\\
\midrule
DualOctreeGNN+AE & 0.14 & 0.038 & 0.067 & 0.695 & 512.0 & 86.069 $\pm$ 6.719 & 51.809 $\pm$ 13.737 \\
DualOctreeGNN+VAE & 0.16 & 0.038 & 0.065 & 0.695 & 512.0 & 85.47 $\pm$ 7.646 & 52.958 $\pm$ 14.539 \\
DualOctreeGNN+VAE+KL & 0.146 & 0.034 & 0.062 & 0.453 & 512.0 & 56.388 $\pm$ 20.291 & 115.326 $\pm$ 47.412 \\
\bottomrule
\end{tabular}
}
\caption{Reconstruction quality (Category: Chair, Dataset: ShapeNet test set) This shows that KL loss degrades the reconstruction quality for the chair category as well.}
\label{tab:reconstruction_dualoctree_chair}
\end{table*}


\begin{table*}[htb]
\caption{Generation quality (ShapeNet, number of samples: 25)}
\label{tab:generation_dualoctree}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
Representation & Epochs & Batch Size & Category &COV $\uparrow$ & MMD$\downarrow$   &1-NNA $\uparrow$ \\
\midrule
DualOctreeGNN+VAE+UNet3D & 900& 112 &Airplane&0.4&0.0226298& 0.9\\
DualOctreeGNN+VAE+UNet3D & 500& 112 &Car&0.04&0.04375737& 0.98\\
DualOctreeGNN+VAE+UNet3D & 500& 224 &Chair&0.2&0.0853681& 1\\
\bottomrule
\end{tabular}
}
 \end{table*}


==> Figures/generalization_table.tex <==

\begin{table}[ht]
\resizebox{\linewidth}{!}{
\begin{tabular}{llll}
\toprule
Method &  F-score (0.0125) $\uparrow$ & CD (*1e-4) $\downarrow$ & NC $\uparrow$\\
\midrule
DualOctree AE & 48.38 \footnotesize{ $\pm$ 11.39} & 0.047 \footnotesize{ $\pm$ 0.02} & 0.677 \footnotesize{ $\pm$ 0.08} \\
NeRF AE & 26.229 \footnotesize{ $\pm$ 11.64} & 0.107 \footnotesize{ $\pm$ 0.04} & 0.589 \footnotesize{ $\pm$ 0.05} \\
SDF AE & \textbf{91.123 \footnotesize{ $\pm$ 6.02}} & \textbf{0.01 \footnotesize{ $\pm$ 0.01} }& \textbf{0.843 \footnotesize{ $\pm$ 0.05}} \\
% SDF VAE 128 & 82.854 \footnotesize{ $\pm$ 6.67} & 0.017 \footnotesize{ $\pm$ 0.0} & 0.798 \footnotesize{ $\pm$ 0.05} \\
Shape2VecSet AE & 75.338 \footnotesize{ $\pm$ 8.87} & 0.022 \footnotesize{ $\pm$ 0.01} & 0.717 \footnotesize{ $\pm$ 0.07} \\
Triplane AE & 41.69 \footnotesize{ $\pm$ 11.57} & 0.073 \footnotesize{ $\pm$ 0.03} & 0.688 \footnotesize{ $\pm$ 0.07} \\
Voxel VAE & 85.602 \footnotesize{ $\pm$ 9.48} & 0.017 \footnotesize{ $\pm$ 0.01} & 0.8 \footnotesize{ $\pm$ 0.05} \\
% Voxel VAE 128 & 92.444 \footnotesize{ $\pm$ 5.87} & 0.008 \footnotesize{ $\pm$ 0.0} & 0.833 \footnotesize{ $\pm$ 0.05} \\
\bottomrule
\end{tabular}
}
% \vspace{-3mm}
\caption{Reconstruction quality in an out-of-distribution task - reconstructing airplanes with a model trained on chairs.}
\label{tab:reconstruction_generalization}
% \vspace{-3mm}
\end{table}

==> Figures/reconstruction_table.tex <==

\begin{table}[b!ht]
\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{llll}
\toprule
 Method & F-score (0.0125) $\uparrow$ & CD (*1e-4) $\downarrow$ & NC $\uparrow$ \\
\midrule
DualOctree VAE & 76.122 \footnotesize{ $\pm$ 13.44} & 0.02 \footnotesize{ $\pm$ 0.01} & 0.766 \footnotesize{ $\pm$ 0.07} \\
NeRF AE & 58.44 \footnotesize{ $\pm$ 13.22} & 0.034 \footnotesize{ $\pm$ 0.02} & 0.723 \footnotesize{ $\pm$ 0.07} \\
SDF AE & \textbf{88.434 \footnotesize{ $\pm$ 6.58}} & \textbf{0.012 \footnotesize{ $\pm$ 0.0}} & \textbf{0.827 \footnotesize{ $\pm$ 0.06}} \\
Shape2VecSet AE & 79.37 \footnotesize{ $\pm$ 17.04} & 0.023 \footnotesize{ $\pm$ 0.02} & 0.776 \footnotesize{ $\pm$ 0.07} \\
Triplane AE & 66.445 \footnotesize{ $\pm$ 16.06} & 0.028 \footnotesize{ $\pm$ 0.02} & 0.759 \footnotesize{ $\pm$ 0.08} \\
Voxel AE & 85.666 \footnotesize{ $\pm$ 10.54} & 0.016 \footnotesize{ $\pm$ 0.01} & 0.787 \footnotesize{ $\pm$ 0.06} \\
\bottomrule
\end{tabular}
}
\caption{Reconstruction quality in terms of CD, F-score, IoU and NC. OOD refers to testing a model on the Airplane category while it was trained on the Chair category.
}
\label{tab:reconstruction}
\end{table}



==> metrics.tex <==
\subsection{Evaluation Metrics}

We use the following metrics for evaluating our approach.
The symmetric Chamfer distance is selected to measure the distance between two point clouds $X$ and $Y$.
\begin{equation}
    \mathrm{CD}(X,Y) = \frac{1}{|X|}\sum_{x\in X} \min_{y\in Y}\Vert x - y \Vert_2^2 + \frac{1}{|Y|}\sum_{y\in Y} \min_{x\in X}\Vert y - x \Vert_2^2.
    \label{eq:cd}
\end{equation}

The F-score is the harmonic mean of precision and recall for a generated mesh $\gG$ and a reference mesh $\gR$. The precision is defined as
\begin{equation}
    P(\tau) = \frac{100}{|\gG|} \sum_{\rvg \in \gG} \left[ \min_{\rvr \in \gR} \left\Vert \rvg-\rvr \right\Vert_2 < \tau \right],
\end{equation}
with $\rvg$ as points sampled on the surface of the generated mesh, $\rvr$ as points sampled from the reference mesh, $\tau$ as a threshold, and $[\cdot]$ as the Iversion bracket.
The recall is defined accordingly as 
\begin{equation}
    R(\tau) = \frac{100}{|\gR|} \sum_{\rvr \in \gR} \left[ \min_{\rvg \in \gG} \left\Vert \rvr-\rvg \right\Vert_2 < \tau \right].
\end{equation}
The final F-score is then computed as
\begin{equation}
    F(\tau) = \frac{2 P(\tau) R(\tau)}{P(\tau)+R(\tau)}.
    \label{eq:fscore}
\end{equation}

To measure the quality of the generated meshes w.r.t. a set of reference meshes we use the metrics Coverage ($\mathrm{COV}$), Minimum matching distance ($\mathrm{MMD}$), and 1-nearest neighbor accuracy ($\text{1-NNA}$).

\begin{equation}
    \mathrm{COV}(S_g, S_r) = \frac{|\{\mathrm{arg\,min}_{Y\in S_r} D(X,Y) | X\in S_g\}|}{|S_r|}.
    \label{eq:cov}
\end{equation}

\begin{equation}
    \mathrm{MMD}(S_g, S_r) = \frac{1}{|S_r|} \sum_{Y\in S_r}\underset{X\in S_g}{\mathrm{min}} D(X,Y).
    \label{eq:mmd}
\end{equation}

\begin{equation}
    \text{1-NNA}(S_g, S_r) = \frac{\sum_{X\in S_g}\mathbb{I}[N_x\in S_g] + \sum_{Y\in S_r} \mathbb{I}[N_y \in S_r]}{|S_g|+|S_r|}.
    \label{eq:1nna}
\end{equation}
$N_X$ is the nearest neighbor of $X$ in the set $S_r \cup S_g - \{X\}$. $S_r$, $S_g$ are the sets of reference and generated meshes and are of equal size.
We use the Chamfer distance for $D$ in all our experiments.



\begin{figure}
    \centering
    \adjustbox{width=\textwidth}{
        \includegraphics[height=3cm]{Figures/unconditional_metrics/ShapenetPreprocessed_airplane_COV_plot.pdf}
        \includegraphics[height=3cm]{Figures/unconditional_metrics/ShapenetPreprocessed_airplane_MMD_plot.pdf}
        \includegraphics[height=3cm]{Figures/unconditional_metrics/ShapenetPreprocessed_airplane_1-NNA_plot.pdf}
    }
    \begin{subfigure}[b]{0.32\textwidth}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
    \caption{}
    \end{subfigure}
    \caption{We select 100 random subsets of different sizes of the train and test split of Shapenet and compute the COV,MMD, and 1-NNA metrics.}
    \label{fig:quality_datasets}
\end{figure}

